Introduction to Homotopy Type Theory

This is an introductory textbook to univalent mathematics and homotopy type theory, a mathematical foundation that takes advantage of the structural nature of mathematical definitions and constructions. It is common in mathematical practice to consider equivalent objects to be the same, for example, to identify isomorphic groups. In set theory it is not possible to make this common practice formal. For example, there are as many distinct trivial groups in set theory as there are distinct singleton sets. Type theory, on the other hand, takes a more structural approach to the foundations of mathematics that accommodates the univalence axiom. This, however, requires us to rethink what it means for two objects to be equal. This textbook introduces the reader to Martin-L\"of's dependent type theory, to the central concepts of univalent mathematics, and shows the reader how to do mathematics from a univalent point of view. Over 200 exercises are included to train the reader in type theoretic reasoning. The book is entirely self-contained, and in particular no prior familiarity with type theory or homotopy theory is assumed.

==> hott.tex <==
% AUTHOR: Egbert Rijke
% LAST MODIFIED: February 2020

\makeatletter


% Display format for sections
%\crefformat{section}{\S#2#1#3}
%\Crefformat{section}{Section~#2#1#3}
%\crefrangeformat{section}{\S\S#3#1#4--#5#2#6}
%\Crefrangeformat{section}{Sections~#3#1#4--#5#2#6}
%\crefmultiformat{section}{\S\S#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\Crefmultiformat{section}{Sections~#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\crefrangemultiformat{section}{\S\S#3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}{, #3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}
%\Crefrangemultiformat{section}{Sections~#3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}{, #3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}

% Display format for appendices
%\crefformat{appendix}{Appendix~#2#1#3}
%\Crefformat{appendix}{Appendix~#2#1#3}
%\crefrangeformat{appendix}{Appendices~#3#1#4--#5#2#6}
%\Crefrangeformat{appendix}{Appendices~#3#1#4--#5#2#6}
%\crefmultiformat{appendix}{Appendices~#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\Crefmultiformat{appendix}{Appendices~#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\crefrangemultiformat{appendix}{Appendices~#3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}{, #3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}
%\Crefrangemultiformat{appendix}{Appendices~#3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}{, #3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}

%\crefname{part}{Part}{Parts}

%\crefformat{paragraph}{\S#2#1#3}
%\Crefformat{paragraph}{Paragraph~#2#1#3}
%\crefrangeformat{paragraph}{\S\S#3#1#4--#5#2#6}
%\Crefrangeformat{paragraph}{Paragraphs~#3#1#4--#5#2#6}
%\crefmultiformat{paragraph}{\S\S#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\Crefmultiformat{paragraph}{Paragraphs~#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\crefrangemultiformat{paragraph}{\S\S#3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}{, #3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}
%\Crefrangemultiformat{paragraph}{Paragraphs~#3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}{, #3#1#4--#5#2#6}{ and~#3#1#4--#5#2#6}

% Display format for figures
%\crefname{figure}{Figure}{Figures}
%\crefname{table}{Table}{Tables}

% Use cleveref instead of hyperref's \autoref
\let\autoref\cref


%%%% EQUATION NUMBERING %%%%

% The following hack uses the single theorem counter to number
% equations as well, so that we don't have both Theorem 1.1 and
% equation (1.1).

%\let\c@equation\c@thm

\numberwithin{equation}{subsection}


%%%% ENUMERATE NUMBERING %%%%

% Number the first level of enumerates as (i), (ii), ...
%\renewcommand{\theenumi}{(\roman{enumi})}
%\renewcommand{\labelenumi}{\theenumi}
% \def\makeRRlabeldot#1{\hss\llap{#1}}
\renewcommand\theenumi{{\rm (\roman{enumi})}}
\renewcommand\theenumii{{\rm (\alph{enumii})}}
\renewcommand\theenumiii{{\rm (\arabic{enumiii})}}
\renewcommand\theenumiv{{\rm (\Alph{enumiv})}}

%%%% CITATIONS %%%%

% \let \cite \citep

%%%% INDEX %%%%

%\newcommand{\footstyle}[1]{{\hyperpage{#1}}n} % If you index something that is in a footnote
%\newcommand{\defstyle}[1]{\textbf{\hyperpage{#1}}}  % Style for pageref to a definition

%%% Term being defined
\newcommand{\define}[1]{\textbf{#1}}
\newcommand{\quasidefine}[1]{\emph{#1}}
\newcommand{\indexdef}[1]{\index{#1|defstyle}}   % Index a definition
\newcommand{\indexfoot}[1]{\index{#1|footstyle}} % Index a term in a footnote
\newcommand{\indexsee}[2]{\index{#1|see{#2}}}    % Index "see also"

%% Use \symlabel instead of \label to mark a pageref that you need in the index of symbols
\newcounter{symindex}
\newcommand{\symlabel}[1]{\refstepcounter{symindex}\label{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% MACROS FOR NOTATION %%%%
% Use these for any notation where there are multiple options.

%%% Definitional equality (used infix) %%%
\newcommand{\jdeq}{\doteq}      % An equality judgment
\newcommand{\defeq}{\coloneqq} %{\vcentcolon\jdeq}  % A judgmental equality currently being defined

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Type constructors and quantifiers

%%% Universal quantification of mere propositions
\newcommand{\fall}[1]{\forall_{(#1)}\,\@ifnextchar\bgroup{\fall}{}}

%%% Existential quantifier %%%
\newcommand{\exis}[1]{\exists_{(#1)}\,\@ifnextchar\bgroup{\exis}{}}

%%% Unique existence %%%
\newcommand{\uexis}[1]{\exists!_{(#1)}\,\@ifnextchar\bgroup{\uexis}{}}

%%% Dependent sums %%%
\def\smsym{\sum}
\newcommand{\@thesum}[1]{\smsym_{(#1)}}
\newcommand{\sm}[1]{\@ifnextchar\bgroup{\@sm{#1}\sm}{\@sm{#1}}}
\newcommand{\@sm}[1]{\mathchoice{{\textstyle\@thesum{#1}}}{\@thesum{#1}}{\@thesum{#1}}{\@thesum{#1}}}

%%% Dependent products %%%
\def\prdsym{\prod}
\newcommand{\@theprd}[1]{\prdsym_{(#1)}}
\newcommand{\prd}[1]{\@ifnextchar\bgroup{\@prd{#1}\prd}{\@prd{#1}}}
\newcommand{\@prd}[1]{\mathchoice{{\textstyle\@theprd{#1}}}{\@theprd{#1}}{\@theprd{#1}}{\@theprd{#1}}}

% \newcommand{\tprd}{\prd}

% Other notations related to dependent sums
\newcommand{\pairr}[1]{{\mathopen{}(#1)\mathclose{}}}
\newcommand{\Pairr}[1]{{\mathopen{}\left(#1\right)\mathclose{}}}
\newcommand{\tup}[2]{(#1,#2)}
\newcommand{\proj}[1]{\ensuremath{\mathsf{pr}_{#1}}\xspace}
\newcommand{\fst}{\ensuremath{\proj1}\xspace}
\newcommand{\snd}{\ensuremath{\proj2}\xspace}

%%%% Dependent products
%\def\prdsym{\mathchoice{{{\textstyle\prod}}}{\prod}{\prod}{\prod}}

%% Call the macro like \prd{x,y:A}{p:x=y} with any number of
%% arguments.  Make sure that whatever comes *after* the call doesn't
%% begin with an open-brace, or it will be parsed as another argument.

%%%% Implicit arguments are possible. In the above example, if x and y are to be
%%%% implicit, then one should write \prd*{x,y:A}{p:x=y}
%%%%
%%%% If one wants to use implicit arguments in the notation for product types,
%%%% a * has to be put before the argument that has to be implicit.
%%%% For example: in $\prd{x:A}*{y:B}{u:P(y)}Q(x,y,u)$, the argument y is
%%%% implicit. Any of the arguments can be made implicit this way.

%%%% First of all, we should make the command \prd search not only for a
%%%% brace, but also for a star. We introduce an auxiliary command that
%%%% determines whether the next character is a star or brace.

% \newcommand{\@ifnextchar@starorbrace}[2]
%   {\@ifnextchar*{#1}{\@ifnextchar\bgroup{#1}{#2}}}

% \newcommand{\@theprd}[1]{\prdsym_{(#1)}}
% \newcommand{\@theiprd}[1]{\prdsym_{\{#1\}}}

%%%% When encountering the \prd command, latex should determine whether it
%%%% should print implicit argument brackets or not.
%%%% First, we have the following switch. Set it to true if implicit arguments
%%%% are desired, or to false if not. Note turning off implicit arguments
%%%% might render some parts of the text harder to comprehend, since in the
%%%% text might appear $f(x)$ where we would have $f(i,x)$ without implicit
%%%% arguments.

% \DeclareOption{implicit_arguments_on}%
%   {\newcommand{\implicitargumentson}{\boolean{true}}}
% \DeclareOption{implicit_arguments_off}%
%   {\newcommand{\implicitargumentson}{\boolean{false}}}

% \ExecuteOptions{implicit_arguments_off}

% \ProcessOptions\relax

% \newcommand{\prd}{\@ifnextchar*{\@iprd}{\@prd}}
% \newcommand{\@prd}[1]
%   {\@ifnextchar@starorbrace
%     {\@tprd{#1}\prd}
%     {\@tprd{#1}}}
% \newcommand{\@tprd}[1]{%
%   \mathchoice{%
%     {{\textstyle\@theprd{#1}}}}{\@theprd{#1}}{\@theprd{#1}}{\@theprd{#1}}}

% \newcommand{\@iprd}[2]{\@ifnextchar@starorbrace%
%   {\@tiprd{#2}\prd}%
%   {\@tiprd{#2}}}
% \newcommand{\@tiprd}[1]{
%   \ifthenelse{\implicitargumentson}
%     {\@@tiprd{#1}}%\@ifnextchar\bgroup{\@tiprd}{}}
%     {\@tprd{#1}}}
% \newcommand{\@@tiprd}[1]{\mathchoice{{\textstyle\@theiprd{#1}}}{\@theiprd{#1}}{\@theiprd{#1}}{\@theiprd{#1}}}

%%% Lambda abstractions.
% Each variable being abstracted over is a separate argument.  If
% there is more than one such argument, they *must* be enclosed in
% braces.  Arguments can be untyped, as in \lam{x}{y}, or typed with a
% colon, as in \lam{x:A}{y:B}. In the latter case, the colons are
% automatically noticed and (with current implementation) the space
% around the colon is reduced.  You can even give more than one variable
% the same type, as in \lam{x,y:A}.
\def\lam#1{{\lambda}\@lamarg#1:\@endlamarg\@ifnextchar\bgroup{.\,\lam}{.\,}}
\def\@lamarg#1:#2\@endlamarg{\if\relax\detokenize{#2}\relax #1\else\@lamvar{\@lameatcolon#2},#1\@endlamvar\fi}
\def\@lamvar#1,#2\@endlamvar{(#2\,{:}\,#1)}
% \def\@lamvar#1,#2{{#2}^{#1}\@ifnextchar,{.\,{\lambda}\@lamvar{#1}}{\let\@endlamvar\relax}}
\def\@lameatcolon#1:{#1}
\let\lamt\lam
% This version silently eats any typing annotation.
\def\lamu#1{{\lambda}\@lamuarg#1:\@endlamuarg\@ifnextchar\bgroup{.\,\lamu}{.\,}}
\def\@lamuarg#1:#2\@endlamuarg{#1}

\mathchardef\usc="2D
%\newcommand{\usc}{\underline{\ }}

% Macros for dependent type theory
\newcommand{\type}{\mathrm{type}}
\newcommand{\Coq}{\textsc{Coq}\xspace}
\newcommand{\Agda}{\textsc{Agda}\xspace}
\newcommand{\NuPRL}{\textsc{NuPRL}\xspace}

% Macros for dependent function types
\newcommand{\idfunc}[1][]{\mathsf{id}_{#1}}
\newcommand{\const}{\mathsf{const}}
\newcommand{\comp}{\mathsf{comp}}
\newcommand{\blank}{\mathord{\hspace{1pt}\text{--}\hspace{1pt}}}
\newcommand{\newdef}{\mathsf{c}}

% Macros for natural numbers
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\zeroN}{0_{\N}}
\newcommand{\oneN}{1_{\N}}
\newcommand{\succN}{\mathsf{succ}_{\N}}
\newcommand{\addN}{\mathsf{add_{\N}}}
\newcommand{\addzeroN}{\mathsf{add\usc{}zero}_\N}
\newcommand{\addsuccN}{\mathsf{add\usc{}succ}_\N}
\newcommand{\addpN}{\mathsf{add'_{\N}}}
\newcommand{\mulN}{\mathsf{mul}_{\N}}
\newcommand{\minN}{\mathsf{min}_{\N}}
\newcommand{\maxN}{\mathsf{max}_{\N}}
\newcommand{\indN}{\ind{\N}}

% Macros for inductive types
\newcommand{\ind}[1]{\mathsf{ind}_{#1}}
\newcommand{\comphtpy}[1]{\mathsf{comp}_{#1}}

\newcommand{\unit}{\ensuremath{\mathbf{1}}\xspace}
\newcommand{\ttt}{\star}
\newcommand{\indunit}{\mathsf{ind}_{\unit}}
\newcommand{\pt}{\mathsf{pt}}

\newcommand{\emptyt}{\emptyset}
\newcommand{\indempty}{\mathsf{ind}_{\emptyt}}
\newcommand{\exfalso}{\mathsf{ex\usc{}falso}}
\newcommand{\isempty}{\mathsf{is\usc{}empty}}

\newcommand{\bool}{\mathsf{bool}}
\newcommand{\btrue}{\mathsf{true}}
\newcommand{\bfalse}{\mathsf{false}}
\newcommand{\bneg}{\mathsf{neg}}
\newcommand{\indbool}{\mathsf{ind\usc{}bool}}
\newcommand{\negbool}{\mathsf{neg\usc{}bool}}

\newcommand{\inlsym}{{\mathsf{inl}}}
\newcommand{\inrsym}{{\mathsf{inr}}}
\newcommand{\inl}{\ensuremath\inlsym\xspace}
\newcommand{\inr}{\ensuremath\inrsym\xspace}
\newcommand{\indcoprod}{\mathsf{ind}_{+}}

\newcommand{\pair}{\mathsf{pair}}
\newcommand{\indSigma}{\mathsf{ind}_{\Sigma}}

\newcommand{\indprod}{\mathsf{ind}_{\times}}

\newcommand{\Z}{{\mathbb{Z}}}
\newcommand{\inpos}{\mathsf{in\usc{}pos}}
\newcommand{\inneg}{\mathsf{in\usc{}neg}}
\newcommand{\indZ}{\mathsf{ind}_{\mathbb{Z}}}
\newcommand{\zeroZ}{0_{\Z}}
\newcommand{\oneZ}{1_{\Z}}
\newcommand{\succZ}{\mathsf{succ}_{\Z}}
\newcommand{\predZ}{\mathsf{pred}_{\Z}}
\newcommand{\addZ}{\mathsf{add}_{\Z}}
\newcommand{\mulZ}{\mathsf{mul}_{\Z}}
\newcommand{\negZ}{\mathsf{neg}_{\Z}}

\newcommand{\lst}{\mathsf{list}}
\newcommand{\nil}{\mathsf{nil}}
\newcommand{\cons}{\mathsf{cons}}
\newcommand{\fold}{\mathsf{fold}}
\newcommand{\foldlist}{\mathsf{fold\usc{}list}}
\newcommand{\maplist}{\mathsf{map\usc{}list}}
\newcommand{\lengthlist}{\mathsf{length\usc{}list}}
\newcommand{\sumlist}{\mathsf{sum\usc{}list}}
\newcommand{\productlist}{\mathsf{product\usc{}list}}
\newcommand{\reverselist}{\mathsf{reverse\usc{}list}}
\newcommand{\concatlist}{\mathsf{concat\usc{}list}}
\newcommand{\flattenlist}{\mathsf{flatten\usc{}list}}

% Macros for identity types
\newcommand{\idsymbin}{=}
\newcommand{\idsym}{{\idsymbin}}
\newcommand{\id}[3][]{
  \@ifnextchar\bgroup
    {#2 \mathbin{\idsym_{#1}} \id[#1]{#3}}
    {#2 \mathbin{\idsym_{#1}} #3}
  }
\newcommand{\idtype}[3][]{\ensuremath{\mathsf{Id}_{#1}(#2,#3)}\xspace}
\newcommand{\idtypevar}[1]{\ensuremath{\mathsf{Id}_{#1}}\xspace}
\newcommand{\refl}[1]{\mathsf{refl}_{#1}}
\newcommand{\pathind}{\mathsf{ind\usc{}eq}}

\newcommand{\concat}{\mathsf{concat}}
\newcommand{\ctsym}{%
  \mathchoice{\mathbin{\raisebox{0.5ex}{$\displaystyle\centerdot$}}}%
             {\mathbin{\raisebox{0.5ex}{$\centerdot$}}}%
             {\mathbin{\raisebox{0.25ex}{$\scriptstyle\,\centerdot\,$}}}%
             {\mathbin{\raisebox{0.1ex}{$\scriptscriptstyle\,\centerdot\,$}}}
  }
\newcommand{\ct}[3][]{
  \@ifnextchar\bgroup
    {#2 \mathbin{\ctsym_{#1}} \ct[#1]{#3}}
    {#2 \mathbin{\ctsym_{#1}} #3}
}

\newcommand{\leftunit}{\mathsf{left\usc{}unit}}
\newcommand{\rightunit}{\mathsf{right\usc{}unit}}
\newcommand{\cohunit}{\mathsf{coh\usc{}unit}}
\newcommand{\invfunc}{\mathsf{inv}}
\newcommand{\leftinv}{\mathsf{left\usc{}inv}}
\newcommand{\rightinv}{\mathsf{right\usc{}inv}}
\newcommand{\cohinv}{\mathsf{coh\usc{}inv}}
\newcommand{\assoc}{\mathsf{assoc}}

\newcommand{\apid}{\mathsf{ap\usc{}id}}
\newcommand{\apcomp}{\mathsf{ap\usc{}comp}}
\newcommand{\aprefl}{\mathsf{ap\usc{}refl}}
\newcommand{\apinv}{\mathsf{ap\usc{}inv}}
\newcommand{\apconcat}{\mathsf{ap\usc{}concat}}

\newcommand{\tr}{\mathsf{tr}}
\newcommand{\mapfunc}[1]{\ensuremath{\mathsf{ap}_{#1}}\xspace}
\newcommand{\map}[2]{\mapfunc{#1}({#2})\xspace}
\let\Ap\map
\newcommand{\mapdepfunc}[1]{\ensuremath{\mathsf{apd}_{#1}}\xspace}
\newcommand{\mapdep}[2]{\ensuremath{\mapdepfunc{#1}\mathopen{}\left(#2\right)\mathclose{}}\xspace}
\let\apfunc\mapfunc
\let\ap\map
\let\apdfunc\mapdepfunc
\let\apd\mapdep

\newcommand{\distributiveinvconcat}{\mathsf{distributive\usc{}inv\usc{}concat}}
\newcommand{\invcon}{\mathsf{inv\usc{}con}}
\newcommand{\coninv}{\mathsf{con\usc{}inv}}
\newcommand{\lift}{\mathsf{lift}}
\newcommand{\leftunitlawaddN}{\mathsf{left\usc{}unit\usc{}law\usc{}add_\N}}
\newcommand{\rightunitlawaddN}{\mathsf{right\usc{}unit\usc{}law\usc{}add_\N}}
\newcommand{\leftsuccessorlawaddN}{\mathsf{left\usc{}successor\usc{}law\usc{}add_\N}}
\newcommand{\rightsuccessorlawaddN}{\mathsf{right\usc{}successor\usc{}law\usc{}add_\N}}
\newcommand{\associativeaddN}{\mathsf{associative\usc{}add_\N}}
\newcommand{\commutativeaddN}{\mathsf{commutative\usc{}add_\N}}

% Macros for universes
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\Ty}{\mathcal{T}}
\newcommand{\EqN}{\mathsf{Eq}_{\N}}
\newcommand{\reflEqN}{\mathsf{refl\usc{}Eq}_\N}
\newcommand{\indEqN}{\mathsf{ind\usc{}Eq}_\N}
\newcommand{\EqBool}{\mathsf{Eq\usc{}bool}}
\newcommand{\universalfam}{\Ty}
\newcommand{\distN}{\mathsf{dist}_\N}
\newcommand{\vect}{\mathsf{vector}}
\newcommand{\mat}{\mathsf{matrix}}
\newcommand{\nilvertical}{\mathsf{nil\usc{}vert}}
\newcommand{\nilhorizontal}{\mathsf{nil\usc{}horiz}}
\newcommand{\consvertical}{\mathsf{cons\usc{}vert}}
\newcommand{\conshorizontal}{\mathsf{cons\usc{}horiz}}
\newcommand{\transpose}{\mathsf{transpose}}

% Macros for modular arithmetic
\newcommand{\cgrN}{\mathsf{cong}_\N}%The congruence relation
\renewcommand{\mod}{\ \ \mathsf{mod}\ }
\newcommand{\Fin}[1]{\ensuremath{\mathsf{Fin}}_{#1}}%The finite sets
\newcommand{\indFin}{\mathsf{ind\usc{}Fin}}
\newcommand{\natFin}{\iota}%The inclusion of finite sets in N
\newcommand{\negtwoFin}{\mathsf{neg\usc{}two}}%-2 in Fin
\newcommand{\negoneFin}{\mathsf{neg\usc{}one\usc}}%-1 in Fin
\newcommand{\zeroFin}{\mathsf{zero}}%0 in Fin
\newcommand{\oneFin}{\mathsf{one}}%1 in Fin
\newcommand{\skipzeroFin}{\mathsf{skip\usc{}zero}}%The function that skips 0
\newcommand{\succFin}{\mathsf{succ}}%The successor function on Fin
\newcommand{\skipnegtwoFin}{\mathsf{skip\usc{}neg\usc{}two}}%The function that skips -2
\newcommand{\predFin}{\mathsf{pred}}%The predecessor function
\newcommand{\EqFin}{\mathsf{Eq}}%Observational equality on Fin
\newcommand{\reflEqFin}{\mathsf{refl\usc{}Eq}}%Reflexivity of observational Eq
\newcommand{\swapFin}{\mathsf{swap}}
\newcommand{\addFin}{\mathsf{add}}
\newcommand{\negFin}{\mathsf{neg}}
\newcommand{\mulFin}{\mathsf{mul}}
\newcommand{\with}{~\mathit{with}~}
\newcommand{\reverseFin}{\mathsf{reverse}}
\newcommand{\skipFin}{\delta}
\newcommand{\repeatFin}{\sigma}
\newcommand{\basedN}[1]{\N_{#1}}
\newcommand{\constantbasedN}[1]{\mathsf{constant}_{\basedN{#1}}}
\newcommand{\unaryopbasedN}[1]{\mathsf{unary\usc{}op}_{\basedN{#1}}}
\newcommand{\EqbasedN}[1]{\mathsf{Eq_{\basedN{k}}}}
\newcommand{\convertbasedN}[1]{f_{#1}}
\newcommand{\isfinitelycyclic}{\mathsf{is\usc{}finitely\usc{}cyclic}}
\newcommand{\issplitsurjective}{\mathsf{is\usc{}split\usc{}surjective}}
\newcommand{\classicalFin}{\mathsf{classical\usc{}Fin}}

% Macros for elementary number theory
\DeclareMathOperator{\lcm}{lcm}
\newcommand{\isdecidable}{\mathsf{is\usc{}decidable}}
\newcommand{\isdec}{\isdecidable}
\newcommand{\hasdecidableequality}{\mathsf{has\usc{}decidable\usc{}eq}}
\newcommand{\collatz}{\mathsf{collatz}}
\newcommand{\decidableProp}{\mathsf{DProp}}
\newcommand{\decunit}{\mathsf{dec}_\unit}
\newcommand{\decemptyt}{\mathsf{dec}_\emptyt}
\renewcommand{\gcd}{\mathsf{gcd}}
\newcommand{\isminimal}{\mathsf{is\usc{}minimal}}
\newcommand{\ismaximal}{\mathsf{is\usc{}maximal}}
\newcommand{\islowerbound}{\mathsf{is\usc{}lower\usc{}bound}}
\newcommand{\isupperbound}{\mathsf{is\usc{}upper\usc{}bound}}
\newcommand{\wellorderingprinciple}{\mathsf{w}}
\newcommand{\ismultipleofgcd}{M}
\newcommand{\isbounded}{\mathsf{is\usc{}bounded}}
\newcommand{\maximum}{\mathsf{maximum}}
\newcommand{\minimum}{\mathsf{minimum}}
\newcommand{\isprime}{\mathsf{is\usc{}prime}}
\newcommand{\strongindN}{\mathsf{strong\usc{}ind}_\N}
\newcommand{\reflleqN}{\mathsf{refl\usc{}leq}_\N}
\newcommand{\ordindN}{\mathsf{ord\usc{}ind}_\N}
\newcommand{\gcdeuclid}{\mathsf{gcd}_E}
\newcommand{\isgcd}{\mathsf{is\usc{}gcd}}
\newcommand{\isproperdivisor}{\mathsf{is\usc{}proper\usc{}divisor}}
\newcommand{\isdecidableisprime}{\mathsf{is\usc{}decidable\usc{}is\usc{}prime}}
\newcommand{\booleanization}{\mathsf{booleanization}}
\newcommand{\booleanreflection}{\mathsf{reflect}}
\let\reflect\booleanreflection
\newcommand{\isprimethirtyseven}{\mathsf{is\usc{}prime\usc{}37}}
\newcommand{\primefunction}{\mathsf{prime}}
\newcommand{\primefactors}{\mathsf{prime\usc{}factors}}
\newcommand{\primeN}{\mathsf{prime}}
\newcommand{\Eqlist}{\mathsf{Eq\usc{}list}}
\newcommand{\invmul}{\mathsf{inv\usc{}mul}}

% Macros for equivalences
\newcommand{\negnegbool}{\mathsf{neg\usc{}neg\usc{}bool}}
\newcommand{\htpy}{\sim}
\newcommand{\reflhtpy}{\mathsf{refl\usc{}htpy}}
\newcommand{\invhtpy}{\mathsf{inv\usc{}htpy}}
\newcommand{\concathtpy}{\mathsf{concat\usc{}htpy}}
\newcommand{\leftunithtpy}{\mathsf{left\usc{}unit\usc{}htpy}}
\newcommand{\rightunithtpy}{\mathsf{right\usc{}unit\usc{}htpy}}
\newcommand{\leftinvhtpy}{\mathsf{left\usc{}inv\usc{}htpy}}
\newcommand{\rightinvhtpy}{\mathsf{right\usc{}inv\usc{}htpy}}
\newcommand{\assochtpy}{\mathsf{assoc\usc{}htpy}}
\newcommand{\sections}{\mathsf{sec}}
\renewcommand{\sec}{\sections}
\newcommand{\retractions}{\mathsf{retr}}
\newcommand{\Retr}{\mathsf{Retr}}
\newcommand{\isequiv}{\mathsf{is\usc{}equiv}}
\newcommand{\eqvsym}{\simeq}    % infix symbol
\newcommand{\eqv}[2]{\@ifnextchar\bgroup{#1 \eqvsym \eqv{#2}}{#1 \eqvsym #2}}
\newcommand{\hasinverse}{\mathsf{has\usc{}inverse}}
\newcommand{\EqSigma}{\mathsf{Eq}_{\Sigma}}
\newcommand{\reflexiveEqSigma}{\mathsf{reflexive\usc{}Eq}_{\Sigma}}
\newcommand{\paireq}{\mathsf{pair\usc{}eq}}
\newcommand{\eqpair}{\mathsf{eq\usc{}pair}}
\newcommand{\assocSigma}{\mathsf{assoc\usc{}}\Sigma}
\newcommand{\swapSigma}{\mathsf{swap\usc{}}\Sigma}
\newcommand{\leftunitlawaddZ}{\mathsf{left\usc{}unit\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\rightunitlawaddZ}{\mathsf{right\usc{}unit\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\leftpredecessorlawaddZ}{\mathsf{left\usc{}predecessor\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\rightpredecessorlawaddZ}{\mathsf{right\usc{}predecessor\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\leftsuccessorlawaddZ}{\mathsf{left\usc{}successor\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\rightsuccessorlawaddZ}{\mathsf{right\usc{}successor\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\assocaddZ}{\mathsf{assoc\usc{}add\usc{}}\Z}
\newcommand{\commaddZ}{\mathsf{comm\usc{}add\usc{}}\Z}
\newcommand{\leftinverselawaddZ}{\mathsf{left\usc{}inverse\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\rightinverselawaddZ}{\mathsf{right\usc{}inverse\usc{}law\usc{}add\usc{}}\Z}
\newcommand{\starvalue}{\mathsf{star\usc{}value}}

% Macros for contractible types
\newcommand{\indsing}{\mathsf{ind\usc{}sing}}
\newcommand{\compsing}{\mathsf{comp\usc{}sing}}
\let\singind\indsing
\let\singcomp\compsing
\newcommand{\evrefl}{\mathsf{ev\usc{}refl}}
\newcommand{\iscontr}{\ensuremath{\mathsf{is\usc{}contr}}}
\newcommand{\ev}{\mathsf{ev}}
\newcommand{\evpt}{\mathsf{ev\usc{}pt}}
\newcommand{\evpair}{\mathsf{ev\usc{}pair}}
\newcommand{\evid}{\mathsf{ev\usc{}id}}
\newcommand{\fibf}[1]{\mathsf{fib}_{#1}}
\newcommand{\fib}[2]{\mathsf{fib}_{#1}(#2)}
\newcommand{\Fib}[2]{\mathsf{fib}_{#1}\left(#2\right)}
\newcommand{\Eqfib}{\mathsf{Eq\usc{}fib}}
\newcommand{\iscohinvertible}{\mathsf{is\usc{}coh\usc{}invertible}}
\newcommand{\nathtpy}{\mathsf{nat\usc{}htpy}}

% Macros for fundamental theorem of identity types
\newcommand{\tot}[2][]{\ensuremath{\mathsf{tot}_{#1}(#2)}}
\newcommand{\isemb}{\mathsf{is\usc{}emb}}
\newcommand{\Eqcoprod}{\mathsf{Eq\usc{}copr}}
\newcommand{\Eqcoprodeq}{\mathsf{Eq\usc{}copr\usc{}eq}}
\newcommand{\cohreduction}{\mathsf{coh\usc{}reduction}}
\newcommand{\fibtriangle}{\mathsf{fib\usc{}triangle}}
\newcommand{\isinj}{\mathsf{is\usc{}inj}}

% Macros for truncation levels
\newcommand{\isprop}{\ensuremath{\mathsf{is\usc{}prop}}}
\newcommand{\prop}{\mathsf{Prop}}
\newcommand{\isset}{\ensuremath{\mathsf{is\usc{}set}}}
\newcommand{\axiomK}{\mathsf{axiom\usc{}K}}
\newcommand{\istrunc}[1]{\mathsf{is\usc{}trunc}_{#1}}
\newcommand{\typele}[1]{\UU^{\leq #1}}
\newcommand{\typeleU}[1]{\ensuremath{{#1}\text-\mathsf{Type}_\UU}\xspace}
\newcommand{\typelep}[1]{\ensuremath{{(#1)}\text-\mathsf{Type}}\xspace}
\newcommand{\typelepU}[1]{\ensuremath{{(#1)}\text-\mathsf{Type}_\UU}\xspace}
\let\ntype\typele
\let\ntypeU\typeleU
\let\ntypep\typelep
\let\ntypepU\typelepU
\newcommand{\set}{\ensuremath{\mathsf{Set}}\xspace}
\newcommand{\setU}{\ensuremath{\mathsf{Set}_\UU}\xspace}
\newcommand{\propU}{\ensuremath{\mathsf{Prop}_\UU}\xspace}
\newcommand{\T}{\mathbb{T}}
\newcommand{\negtwoT}{-2_{\T}}
\newcommand{\succT}{\mathsf{succ}_{\T}}
\newcommand{\isisolated}{\mathsf{is\usc{}isolated}}

% Macros for function extensionality
\newcommand{\eqhtpy}{\mathsf{eq\usc{}htpy}}
\newcommand{\htpyeq}{\mathsf{htpy\usc{}eq}}
\newcommand{\funext}{\mathsf{funext}}
\newcommand{\evtruefalse}{\mathsf{ev\usc{}true\usc{}false}}
\newcommand{\evunit}{\mathsf{ev\usc{}unit}}
\newcommand{\precomp}[1]{{#1}^\ast}
\newcommand{\pathsplit}{\mathsf{is\usc{}path\usc{}split}}
\newcommand{\choice}{\mathsf{choice}}
\newcommand{\isinvertible}{\mathsf{is\usc{}invertible}}
\newcommand{\evinlinr}{\mathsf{ev\usc{}inl\usc{}inr}}
\newcommand{\homslice}{\mathsf{hom}}

% Macros for univalence
\newcommand{\eqequiv}{\mathsf{eq\usc{}equiv}}
\newcommand{\equiveq}{\mathsf{equiv\usc{}eq}}
\newcommand{\univalence}{\ensuremath{\mathsf{univalence}}\xspace} % the full axiom
\newcommand{\ptdeqvsym}{\simeq_\ast}    % infix symbol
\newcommand{\ptdeqv}[2]{
  \@ifnextchar\bgroup
    {#1 \ptdeqvsym \ptdeqv{#2}}
    {#1 \ptdeqvsym #2}
}
\newcommand{\isfunction}{\mathsf{is\usc{}function}}
\newcommand{\iffeq}{\mathsf{iff\usc{}eq}}
\newcommand{\opp}[1]{#1^{\mathsf{op}}}
\newcommand{\graph}{\mathsf{graph}}
\newcommand{\iffprop}{\leftrightarrow}
\newcommand{\ac}{\mathsf{ac}}
\newcommand{\AC}{\mathsf{AC}}
\newcommand{\LEM}{\mathsf{LEM}}
\newcommand{\preord}{\mathsf{PreOrd}}
\newcommand{\posetreflection}[1]{\trunc{\mathsf{Pos}}{#1}}
\newcommand{\issmall}{\mathsf{is\usc{}small}}
\newcommand{\islocallysmall}{\mathsf{is\usc{}locally\usc{}small}}
\newcommand{\isdecidableemb}{\mathsf{is\usc{}decidable\usc{}emb}}

% Macros for propositional truncation
\newcommand{\issurj}{\mathsf{is\usc{}surj}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\BS}{BS}
\newcommand{\carthomFam}{\mathsf{cart\usc{}hom\usc{}Fam}}
\newcommand{\indbrck}{\mathsf{ind\usc{}ptrunc}}
\newcommand{\isfinite}{\mathsf{is\usc{}finite}}
\newcommand{\BAut}{\mathsf{BAut}}
\newcommand{\isweaklyconstant}{\mathsf{is\usc{}weakly\usc{}constant}}
\newcommand{\brckcheck}[1]{\brck{#1}\,\check{}\,}
\newcommand{\source}{\mathsf{source}}
\newcommand{\target}{\mathsf{target}}
\newcommand{\pathI}{\mathsf{path}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\numberofelements}{\mathsf{number\usc{}of\usc{}elements}}
\DeclareRobustCommand{\stirling}{\genfrac\{\}{0pt}{}}

% Macros for finite types
\newcommand{\cnt}{\mathsf{count}}
\renewcommand{\complement}[1]{{#1}^{\mathsf{c}}}
\newcommand{\fallingfactorial}[2]{(#1)_{#2}}
\newcommand{\numberofsurjectivemaps}[2]{\mathsf{S}(#1,#2)}

% Macros for groups in univalent mathematics
\DeclareMathOperator{\Aut}{Aut}
\newcommand{\hasassociativemul}{\mathsf{has\usc{}associative\usc{}mul}}
\newcommand{\semigroup}{\mathsf{Semigroup}}
\newcommand{\monoid}{\mathsf{Monoid}}
\newcommand{\group}{\mathsf{Group}}
\newcommand{\isunital}{\mathsf{is\usc{}unital}}
\newcommand{\isgroup}{\mathsf{is\usc{}group}}
\renewcommand{\hom}{\mathsf{hom}}
\newcommand{\isiso}{\mathsf{is\usc{}iso}}
\newcommand{\isoeq}{\mathsf{iso\usc{}eq}}
\newcommand{\iso}{\mathsf{iso}}
\newcommand{\Set}{\mathsf{Set}}
\newcommand{\binomtype}{\binom}
\newcommand{\dbinomtype}[3][]{\binom{#2}{#3}_{#1}}
\newcommand{\demb}{\hookrightarrow_{\mathsf{d}}}
\newcommand{\emb}{\hookrightarrow}

% Macros for set quotients
\newcommand{\eqrel}{\mathsf{Eq\usc{}Rel}}
\newcommand{\isequivalenceclass}{\mathsf{is\usc{}equivalence\usc{}class}}
\newcommand{\ispartition}{\mathsf{is\usc{}partition}}
\newcommand{\partition}{\mathsf{Partition}}
\newcommand{\isweaklypathconstant}{\mathsf{is\usc{}weakly\usc{}path\usc{}constant}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\ischoiceofrepresentatives}{\mathsf{is\usc{}choice\usc{}of\usc{}reps}}

% Macros for the circle
\newcommand{\gen}{\mathsf{gen}}
\newcommand{\dgen}{\mathsf{dgen}}
\newcommand{\mulcircle}{\mathsf{mul}_{\sphere{1}}}
\newcommand{\basemulcircle}{\mathsf{base\usc{}mul}_{\sphere{1}}}
\newcommand{\loopmulcircle}{\mathsf{loop\usc{}mul}_{\sphere{1}}}
\newcommand{\htpyidcircle}{H}
\newcommand{\basehtpyidcircle}{\alpha}
\newcommand{\loophtpyidcircle}{\beta}
\newcommand{\invcircle}{\mathsf{inv}_{\sphere{1}}}
\newcommand{\evbase}{\mathsf{ev\usc{}base}}
\newcommand{\segmenthelix}{\mathsf{segment\usc{}helix}}
\newcommand{\universalcovercircle}{\mathcal{E}_{\sphere{1}}}

% Macros for the fundamental cover of the circle

% Macros for pullbacks
\newcommand{\ispullback}{\mathsf{is\usc{}pullback}}
\newcommand{\cone}{\mathsf{cone}}
\newcommand{\conemap}{\mathsf{cone\usc{}map}}
\newcommand{\gap}{\mathsf{gap}}
\newcommand{\fibsquare}{\mathsf{fib\usc{}sq}}

% Macros for pushouts
\newcommand{\cocone}{\mathsf{cocone}}
\newcommand{\coconemap}{\mathsf{cocone\usc{}map}}
\newcommand{\gluesym}{{\mathsf{glue}}}
\newcommand{\jglue}{\ensuremath\gluesym\xspace}
\newcommand{\glue}{\mathsf{glue}}
\newcommand{\susp}{\Sigma}
\newcommand{\suspspec}{\susp^\infty}
\newcommand{\north}{\mathsf{N}}
\newcommand{\south}{\mathsf{S}}
\newcommand{\merid}{\mathsf{merid}}
\newcommand{\sphere}[1]{\mathbf{S}^{#1}}
\newcommand{\Sn}{\mathbf{S}}
\newcommand{\base}{\ensuremath{\mathsf{base}}\xspace}
\newcommand{\lloop}{\ensuremath{\mathsf{loop}}\xspace}
\newcommand{\smashpr}[2]{#1 \wedge #2}
\newcommand{\wedgepr}[2]{#1 \vee #2}
\newcommand{\cuppr}[2]{#1 \mathbin{\cupsym} #2}
\newcommand{\cupsym}{\smallsmile}

% Macros for sequential colimits
\newcommand{\seqin}{\mathsf{in\usc{}seq}}
\newcommand{\inseq}{\mathsf{in\usc{}seq}}

% Macros for connected types
\newcommand{\isconn}{\mathsf{is\usc{}conn}}

% Macros for long exact sequences
\newcommand{\mulsphere}[1]{\mathsf{mul}_{\sphere{#1}}}

% Macros for undirected graphs

\newcommand{\unorderedpair}{\mathsf{unordered\usc{}pair}}
\newcommand{\unorderedtuple}{\mathsf{unordered\usc{}tuple}}
\newcommand{\digraph}{\mathsf{Directed\usc{}Graph}}
\newcommand{\undirectedgraph}{\mathsf{Undirected\usc{}Graph}}

% Macros for univalent combinatorics

\newcommand{\intercalate}{\mathsf{intercalate}}
\newcommand{\latinsquare}{\mathsf{Latin\usc{}Square}}

% Macros for later parts of the book

\newcommand{\cart}{\mathsf{cart}}
\newcommand{\esssmall}{\mathsf{ess\usc{}small}}
\newcommand{\locsmall}{\mathsf{loc\usc{}small}}
\newcommand{\isclassified}{\mathsf{is\usc{}classified}}
\newcommand{\tottriangle}{\mathsf{tot\usc{}triangle}}
\newcommand{\idp}{\mathsf{id}^\ast}
\newcommand{\FibSeq}{\mathsf{Fib\usc{}Seq}}
\newcommand{\equivpt}{\mathsf{equiv\usc{}pt}}
\newcommand{\ptequiv}{\mathsf{pt\usc{}equiv}}
\newcommand{\truncunit}[1]{|#1|}
\DeclareMathOperator{\im}{im} % the image
\newcommand{\leftwhisker}{\mathbin{{\ct}_{\ell}}}
\newcommand{\rightwhisker}{\mathbin{{\ct}_{r}}}
\newcommand{\hct}{\star}
\newcommand{\quotientrestr}{\mathsf{quotient\usc{}restriction}}
\newcommand{\pcttype}[2]{\mathsf{Type}_{#1}^{#2}}
\newcommand{\ft}{\sigma}
\newcommand{\bd}{\tau}
\newcommand{\GSet}[1][G]{#1\mathsf{\usc{}Set}}
\newcommand{\Grp}{\mathsf{Group}}
\newcommand{\sslash}{/\mkern-6mu/}
\newcommand{\EM}{\mathsf{EM}}
\newcommand{\iskuratowskyfinite}{\mathsf{is\usc{}kuratowsky\usc{}finite}}
\newcommand{\unorderedpairs}{\mathsf{unordered\usc{}pairs}}
\newcommand{\ispifinite}[1]{\mathsf{is\usc{}}\pi_{#1}\mathsf{\usc{}finite}}
\newcommand{\Tree}{\mathsf{Tree}}
\newcommand{\partitiontype}{\mathsf{Partition\usc{}Type}}
\newcommand{\ferrersdiagram}{\mathsf{Ferrers\usc{}Diagram}}
\newcommand{\isproper}{\mathsf{is\usc{}proper}}
\newcommand{\cycle}{\mathsf{Cycle}}
\newcommand{\polygon}{\mathsf{Polygon}}
\newcommand{\blockdecomposition}{\mathsf{Decomposition}}
\newcommand{\walk}{\mathsf{walk}}
\newcommand{\trail}{\mathsf{trail}}
\newcommand{\Sigmadecomposition}{\Sigma\mathsf{\usc{}decomp}}
\newcommand{\indecomposabletype}{\mathsf{Indecomposable\usc{}Type}}

% Macros for W-types
\newcommand{\M}{\mathbb{M}}
\newcommand{\supW}{\collect}
\newcommand{\collect}{\tree}
\newcommand{\tree}{\mathsf{tree}}
\newcommand{\wcollect}[2]{[ #1\mid #2]}
\newcommand{\Wcollect}[2]{\left[ #1 \mid #2 \right]}
\newcommand{\ecollect}[2]{\{ #1\mid #2\}}
\newcommand{\Ecollect}[2]{\left\{ #1\mid #2\}}
\newcommand{\W}{\mathsf{W}}
\newcommand{\indW}{\mathsf{ind_W}}
\newcommand{\EqW}{\mathsf{Eq_W}}
\newcommand{\reflEqW}{\mathsf{refl\usc{}Eq_W}}
\newcommand{\hasrank}{\mathsf{has\usc{}rank}}
\newcommand{\issmallmultiset}[1]{\mathsf{is\usc{}small_{\M_{#1}}}}
\newcommand{\multiset}[1]{\mathbb{M}_{#1}}
\newcommand{\BinTree}{\mathsf{Bin\usc{}Tree}}
\newcommand{\leaf}{\mathsf{leaf}}
\newcommand{\node}{\mathsf{node}}
\newcommand{\collectBinTree}{\mathsf{bin\usc{}tree}}
\newcommand{\planarBinTree}{\mathbf{T}_2}
\newcommand{\arity}{\mathsf{arity}}
\newcommand{\component}{\mathsf{component}}
\newcommand{\symbolW}{\mathsf{symbol}}
\newcommand{\prearity}{\symbolW}
\newcommand{\rank}{\mathcal{R}}
\newcommand{\isconstantW}{\mathsf{is\usc{}constant_W}}
\newcommand{\yggdrasil}[1][\UU]{\mathbb{Y}_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Basic types

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Universes, subuniverses and modal operators


%Pointed types
\newcommand{\pointed}[1]{\ensuremath{#1_\bullet}}
%%% (pointed) mapping spaces
\newcommand{\Map}{\mathsf{Map}}


\newcommand{\trunc}[2]{\Vert #2\Vert_{#1}}
\newcommand{\Trunc}[2]{\Big\Vert #2\Big\Vert_{#1}}
\newcommand{\truncf}[1]{\Vert \blank \Vert_{#1}}
\newcommand{\tproj}[3][]{\mathopen{}\left|#3\right|_{#2}^{#1}\mathclose{}}
\newcommand{\tprojf}[2][]{|\blank|_{#2}^{#1}}
\def\pizero{\trunc0}
\newcommand{\brck}[1]{\trunc{}{#1}}
\newcommand{\Brck}[1]{\Trunc{}{#1}}
\newcommand{\bproj}[1]{\tproj{}{#1}}
\newcommand{\bprojf}{\tprojf{}}

%%% modalities %%%
\newcommand{\modal}{\ensuremath{\ocircle}}
\newcommand{\modaltype}{\ensuremath{\type_\modal}}
\newcommand{\modalUU}{\ensuremath{\UU_\modal}}
% \newcommand{\ism}[1]{\ensuremath{\mathsf{is}_{#1}}}
% \newcommand{\ismodal}{\ism{\modal}}
% \newcommand{\existsmodal}{\ensuremath{{\exists}_{\modal}}}
% \newcommand{\existsmodalunique}{\ensuremath{{\exists!}_{\modal}}}
% \newcommand{\modalfunc}{\textsf{\modal-fun}}
% \newcommand{\Ecirc}{\ensuremath{\mathsf{E}_\modal}}
% \newcommand{\Mcirc}{\ensuremath{\mathsf{M}_\modal}}
\newcommand{\mreturn}{\ensuremath{\eta}}
\let\project\mreturn
%\newcommand{\mbind}[1]{\ensuremath{\hat{#1}}}
\newcommand{\ext}{\mathsf{ext}}
%\newcommand{\mmap}[1]{\ensuremath{\bar{#1}}}
%\newcommand{\mjoin}{\ensuremath{\mreturn^{-1}}}
% Subuniverse
\renewcommand{\P}{\ensuremath{\type_{P}}\xspace}
\newcommand{\islocal}[1]{\mathsf{is\usc{}local}_{#1}}
\newcommand{\modalunit}[1][]{{\eta_{#1}}}
\newcommand{\plus}[1]{{{#1}^+}}
\newcommand{\localization}[1]{\mathcal{L}_{#1}}
\newcommand{\ismodal}{\ensuremath{\mathsf{is\usc{}modal}}}
\newcommand{\natunit}{\mathsf{nat\usc{}unit}}
\newcommand{\isetale}{\mathsf{is\usc{}etale}}
\newcommand{\etmap}{\mathsf{etale\usc{}map}}

% Projection and extension for truncations
\let\extendsmb\ext
\newcommand{\extend}[1]{\extendsmb(#1)}

%%% Ordinals and cardinals
\newcommand{\card}{\ensuremath{\mathsf{Card}}\xspace}
\newcommand{\ord}{\ensuremath{\mathsf{Ord}}\xspace}
\newcommand{\ordsl}[2]{{#1}_{/#2}}

%%% Some categories
\newcommand{\uset}{\ensuremath{\mathcal{S}et}\xspace}
\newcommand{\ucat}{\ensuremath{{\mathcal{C}at}}\xspace}
\newcommand{\urel}{\ensuremath{\mathcal{R}el}\xspace}
\newcommand{\uhilb}{\ensuremath{\mathcal{H}ilb}\xspace}
\newcommand{\utype}{\ensuremath{\mathcal{T}\!ype}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Miscellaneous stuff

\newcommand{\fibration}{\twoheadrightarrow}
\newcommand{\Sq}[1]{\mathrm{Sq}^{#1}}


% Function definition with domain and codomain
\newcommand{\function}[4]{\left\{\begin{array}{rcl}#1 &
      \longrightarrow & #2 \\ #3 & \longmapsto & #4 \end{array}\right.}


\newcommand{\Hq}{\mathbb{H}}
\newcommand{\Oc}{\mathbb{O}}
\newcommand{\rprojective}[1]{\mathbb{R}\mathsf{P}^{#1}}
\newcommand{\cprojective}[1]{\mathbb{C}\mathsf{P}^{#1}}
\newcommand{\hprojective}[1]{\mathbb{H}\mathsf{P}^{#1}}
\newcommand{\oprojective}[1]{\mathbb{O}\mathsf{P}^{#1}}
\newcommand{\antipodal}[1]{\mathsf{antipodal}_{#1}}


%%% Nameless objects
\newcommand{\nameless}{\mathord{\hspace{1pt}\underline{\hspace{1ex}}\hspace{1pt}}}

\newcommand{\mentalpause}{\medskip} % Use for "mental" pause, instead of \smallskip or \medskip


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% The following is a big unorganized list of new macros that we use in the
%%%% notes. 

\newcommand{\tfW}{\mathsf{W}}
\newcommand{\tfM}{\mathsf{M}}
\newcommand{\mfM}{\modelfont{M}}
\newcommand{\mfN}{\modelfont{N}}
\newcommand{\tfctx}{\mathsf{ctx}}
\newcommand{\mftypfunc}[1]{{\modelfont{typ}^{#1}}}
\newcommand{\mftyp}[2]{{\mftypfunc{#1}(#2)}}
\newcommand{\tftypfunc}[1]{{\mathsf{typ}^{#1}}}
\newcommand{\tftyp}[2]{{\tftypfunc{#1}(#2)}}
\newcommand{\hfibfunc}[1]{\mathsf{fib}_{#1}}
\newcommand{\mappingcone}[1]{\mathcal{C}_{#1}}
\newcommand{\equifib}{\mathsf{equiFib}}
\newcommand{\eqfop}{\mathsf{EqF}}
\newcommand{\eqf}[1]{\eqfop(#1)}
\newcommand{\tfcolim}{\mathsf{colim}}
\newcommand{\colim}{\mathsf{colim}}
\renewcommand{\lim}{\mathsf{lim}}
\newcommand{\tflim}{\mathsf{lim}}
\newcommand{\tfdiag}{\mathsf{diag}}
\newcommand{\tfGraph}{\mathsf{Graph}}
\newcommand{\mfGraph}{\modelfont{Graph}}
\newcommand{\unitGraph}{\unit^\mfGraph}
\newcommand{\UUGraph}{\UU^\mfGraph}
\newcommand{\tfrGraph}{\mathsf{rGraph}}
\newcommand{\mfrGraph}{\modelfont{rGraph}}
\newcommand{\tflimits}{\mathsf{limits}}
\newcommand{\tfcolimits}{\mathsf{colimits}}
\newcommand{\islimiting}{\mathsf{is\usc{}limiting}}
\newcommand{\iscolimiting}{\mathsf{is\usc{}colimiting}}
\newcommand{\islimit}{\mathsf{is\usc{}limit}}
\newcommand{\iscolimit}{\mathsf{is\usc{}colimit}}
\newcommand{\pbcone}{\mathsf{cone_{pb}}}
\newcommand{\tfinj}{\mathsf{inj}}
\newcommand{\tfsurj}{\mathsf{surj}}
\newcommand{\tfepi}{\mathsf{epi}}
\newcommand{\tftop}{\mathsf{top}}
%\newcommand{\sbrck}[1]{\Vert #1\Vert}
%\newcommand{\strunc}[2]{\Vert #2\Vert_{#1}}
\newcommand{\gobjclass}{{\mathsf{U}^\mfGraph}}
\newcommand{\gcharmap}{\mathsf{fib}}
\newcommand{\diagclass}{\mathsf{T}}
\newcommand{\opdiagclass}{\op{\diagclass}}
\newcommand{\equifibclass}{\diagclass^{\eqv{}{}}}
\newcommand{\universe}{\mathsf{U}}
\newcommand{\catid}[1]{{\catfont{id}_{#1}}}
\newcommand{\isleftfib}{\mathsf{is\usc{}left\usc{}fib}}
\newcommand{\isrightfib}{\mathsf{is\usc{}right\usc{}fib}}
\newcommand{\leftLiftings}{\mathsf{leftLiftings}}
\newcommand{\rightLiftings}{\mathsf{rightLiftings}}
\newcommand{\psh}{\mathsf{Psh}}
\newcommand{\rgclass}{\mathsf{\Omega^{RG}}}
\newcommand{\terms}[2][]{| #2 |^{#1}}
\newcommand{\grconstr}[2]
             {\mathchoice % max size is textstyle size.
             {{\textstyle \int_{#1}}#2}% 
             {\int_{#1}#2}%
             {\int_{#1}#2}%
             {\int_{#1}#2}}
\newcommand{\ctxhom}[3][]{\mathsf{hom}_{#1}(#2,#3)}
\newcommand{\graphcharmapfunc}[1]{\gcharmap_{#1}}
\newcommand{\graphcharmap}[2][]{\graphcharmapfunc{#1}(#2)}
\newcommand{\tfexp}[1]{\mathsf{exp}_{#1}}
\newcommand{\tffamfunc}{\mathsf{fam}}
\newcommand{\tffam}[1]{\tffamfunc(#1)}
\newcommand{\tfev}{\mathsf{ev}}
\newcommand{\tfcomp}{\mathsf{comp}}
\newcommand{\smal}{\mathcal{S}}
\renewcommand{\modal}{{\ensuremath{\ocircle}}}
\newcommand{\piw}{\ensuremath{\Pi\mathsf{W}}} %% to be used in conjunction with -pretopos.
%\renewcommand{\sslash}{/\!\!/}
\newcommand{\mprd}[3][]{\Pi^{#1}(#2,#3)}
\newcommand{\msmsym}{\Sigma}
\newcommand{\msm}[2]{\msmsym(#1,#2)}
\newcommand{\mw}[2]{\wtypesym(#1,#2)}
\newcommand{\midt}[1]{\idvartype_#1}
\newcommand{\reflf}[1]{\mathsf{refl}^{#1}}
\newcommand{\tfJ}{\mathsf{J}}
\newcommand{\tftrans}{\mathsf{trans}}
\newcommand{\shapem}{\mathop{\textesh}}

\newcommand{\@gcomp}{\underline}
\newcommand{\gcomp}[1]{{
\renewcommand{\msmsym}{\@gcomp{\Sigma}}
\def\idtypevar##1{\@gcomp{\mathsf{Id}}_{##1}}
\renewcommand{\unit}{\@gcomp{\mathbf{1}}}
\renewcommand{\wtypesym}{\@gcomp{\mathsf{W}}}
\def\reflf##1{\@gcomp{\mathsf{refl}}^{##1}}
#1}}

\newcommand{\tfT}{\mathsf{T}}
\newcommand{\reflsym}{{\mathsf{refl}}}
\newcommand{\strans}[2]{\ensuremath{{#1}_{*}({#2})}}
\newcommand{\eqtype}[1]{\mathsf{Eq}_{#1}}
\newcommand{\eqtoid}[1]{\mathsf{eqtoid}(#1)}
\newcommand{\greek}{\mathrm}
\newcommand{\product}[2]{{#1}\times{#2}}
\newcommand{\pairp}[1]{(#1)}
\newcommand{\jequalizer}[3]{\{#1|#2\jdeq #3\}}
\newcommand{\jequalizerin}[2]{\iota_{#1,#2}}
\newcommand{\tounit}[1]{{!_{#1}}}
\newcommand{\trwk}{\mathsf{trwk}}
\newcommand{\trext}{\mathsf{trext}}
\newcommand{\tfindf}[2][]{\mathsf{ind}_{#2}^{#1}}
\newcommand{\thom}[2]{\mathrm{thom}(#1,#2)}
\newcommand{\thomd}[3]{\mathrm{thom}_{#1}(#2,#3)}

\newcommand{\tfind}[3][]{\tfindf[#1]{#2}(\default@ctxext #3)}
\newcommand{\famtoequifib}{\mathsf{famToEquifib}}
\newcommand{\struct}[1]{\mathop{#1\textnormal{-Struct}}}
\newcommand{\loopspacesym}{\Omega}
\newcommand{\loopspace}[2][]{\loopspacesym^{#1}(#2)}
\newcommand{\join}[3][]{{#2}\ast_{#1}{#3}}
\newcommand{\bigjoinsym}{\mathop{{\scalebox{2.2}{\raisebox{-0.2ex}{$\ast$}}}}}
\newcommand{\@bigjoin}[2]{\bigjoinsym_{(#1)}\,#2}
\newcommand{\bigjoin}[2]{\mathchoice{\textstyle{\@bigjoin{#1}{#2}}}{\@bigjoin{#1}{#2}}{\@bigjoin{#1}{#2}}{\@bigjoin{#1}{#2}}}
\newcommand{\higherequifibsf}{\mathcal}
\newcommand{\higherequifib}[2]{\higherequifibsf{#1}(#2)}
\newcommand{\underlyinggraph}[1]{U(#1)}
\newcommand{\theequifib}[1]{{\def\higherequifibsf{}#1}}
\newcommand{\apbinary}{\mathsf{ap\usc{}binary}}
\newcommand{\subgroup}{\mathsf{Subgroup}}
\newcommand{\concretesubgroup}{\mathsf{Concrete\usc{}Subgroup}}
\newcommand{\concretegroup}{\mathsf{Concrete\usc{}Group}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Categories

\newcommand{\inv}[1]{{#1}^{-1}}
\newcommand{\idtoiso}{\ensuremath{\mathsf{idtoiso}}\xspace}
\newcommand{\isotoid}{\ensuremath{\mathsf{isotoid}}\xspace}
\newcommand{\op}[1]{{{#1}^\mathsf{op}}}
\newcommand{\y}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\dgr}[1]{{#1}^{\dagger}}
\newcommand{\unitaryiso}{\mathrel{\cong^\dagger}}
\newcommand{\cteqv}[2]{\ensuremath{#1 \simeq #2}\xspace}
\newcommand{\cteqvsym}{\simeq}     % Symbol for equivalence of categories

%%% Arrows
\newcommand{\epi}{\ensuremath{\twoheadrightarrow}}
\newcommand{\mono}{\ensuremath{\rightarrowtail}}

%%% Macros for HITs
\newcommand{\cc}{\mathsf{c}}
\newcommand{\pp}{\mathsf{p}}
\newcommand{\cct}{\widetilde{\mathsf{c}}}
\newcommand{\ppt}{\widetilde{\mathsf{p}}}
\newcommand{\Wtil}{\ensuremath{\widetilde{W}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Set theory

\newcommand{\vset}{\mathsf{set}}  % point constructor for cummulative hierarchy V
\def\cd{\tproj0}
\newcommand{\inj}{\ensuremath{\mathsf{inj}}} % type of injections
\newcommand{\acc}{\ensuremath{\mathsf{acc}}} % accessibility

\newcommand{\atMostOne}{\mathsf{atMostOne}}

\newcommand{\power}[1]{\mathcal{P}(#1)} % power set
\newcommand{\powerp}[1]{\mathcal{P}_+(#1)} % inhabited power set

\newcommand{\ucomp}[1]{\hat{#1}}
\newcommand{\fin}{\mathsf{Fin}}
\newcommand{\finsetf}{\mathsf{Fin}}
\newcommand{\finset}[1]{\finsetf(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Group theory

\newcommand{\symmetric}[1]{S_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Introducing logical usage of fonts.
\newcommand{\modelfont}{\mathit} % use 'mf' in command to indicate model font
\newcommand{\catfont}{\mathrm} % use 'cf' in command to indicate cat font

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% When investigation pointed structures we use the \pt macro.

\newcommand*{\bN}{{\mathbb{N}}}
\newcommand*{\bF}{{\mathbb{F}}}
\newcommand*{\bZ}{{\mathbb{Z}}}
\newcommand*{\bR}{{\mathbb{R}}}
\newcommand*{\bC}{{\mathbb{C}}}
\newcommand*{\bH}{{\mathbb{H}}}
\newcommand*{\bS}{{\mathbb{S}}}
\newcommand*{\RP}{{\mathbb{R}\mathrm{P}}}
\newcommand*{\CP}{{\mathbb{C}\mathrm{P}}}
\newcommand*{\HP}{{\mathbb{H}\mathrm{P}}}
\newcommand*{\GType}{\mathrm{GType}} % (k-tuply groupal) n-types
\newcommand*{\nGrp}{\mathrm{\texthyphen Group}} % higher groups
\newcommand*{\Group}{\group}
\newcommand*{\AbGroup}{\mathrm{AbGroup}}
\newcommand*{\iDecat}{\mathrm{\infty\text{-}\mathrm{Decat}}}
\newcommand*{\iDisc}{\mathrm{\infty\text{-}\mathrm{Disc}}}
\newcommand*{\leanref}[1]{}
\newcommand*{\ditto}{--- \raisebox{-0.5ex}{''} ---}
\newcommand*\Sym{S}
\DeclareMathOperator\B{B}
%\newcommand*\BS{\mathop{BS}} 
\newcommand*{\dblslash}{\mathbin{/\kern-3pt/}}
\DeclareMathOperator\Th{Th}
\DeclareMathOperator\Decat{Decat}
\DeclareMathOperator\Disc{Disc}
\DeclareMathOperator\aut{Aut}
\DeclarePairedDelimiter\angled{\langle}{\rangle}
\newcommand{\texthyphen}{\text{-}}
\newcommand{\kersym}{\mathcal{K}}
\newcommand{\qsym}{\mathcal{Q}}
\mathchardef\hyph="2D
\newcommand{\kshiftequiv}{\mathsf{kshift\underline{~}equiv}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\prekersym}{k}

\newcommand{\pto}{\to_{\ast}}
\newcommand{\suspsym}{\Sigma}
\newcommand{\lra}       {\longrightarrow}
\newcommand{\LLL}{\mathcal{L}}
\newcommand{\RRR}{\mathcal{R}}
\newcommand{\sto}{\!\to\!}
\newcommand{\degg}{\mathsf{deg}}
\newcommand{\llra}[1]   {\stackrel{#1}{\lra}}  % labelled long right arrow
\newcommand{\longhookrightarrow}{\lhook\joinrel\lra}
\newcommand{\open}[1]{\mathsf{Op}_{#1}}
\newcommand{\closed}[1]{\mathsf{Cl}_{#1}}
\newcommand{\truncmod}[1]{\mathcal{T}_{#1}}
\newcommand{\shmod}[1]{\mathcal{S}\mathit{h}_{#1}}

\newcommand{\fillers}[1]{\mathsf{fill}_{\mathcal{L},\mathcal{R}}(#1)}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\rsu}[1][\UU]{\mathsf{RSU}_{#1}}
\newcommand{\mdl}[1][\UU]{\mathsf{Mdl}_{#1}}
\newcommand{\lex}[1][\UU]{\mathsf{Lex}_{#1}}
\newcommand{\tpl}[1][\UU]{\mathsf{Top}_{#1}}
\newcommand{\accrsu}[1][\UU]{\mathsf{AccRSU}_{#1}}
\newcommand{\accmdl}[1][\UU]{\mathsf{AccMdl}_{#1}}
\newcommand{\acclex}[1][\UU]{\mathsf{AccLex}_{#1}}

\newcommand{\rcoeq}{\mathsf{rcoeq}}

\newcommand{\tftmfunc}{\mathsf{tm}}
\newcommand{\tftm}[1]{\tftmfunc(#1)}

\DeclarePairedDelimiter\norm{\lVert}{\rVert}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Some tikz macros to typeset diagrams uniformly.

\tikzcdset{arrow style=math font}
\tikzset{patharrow/.style={double,double equal sign distance,-,font=\scriptsize}}
\tikzset{description/.style={fill=white,inner sep=2pt}}
\tikzset{fib/.style={->>,font=\scriptsize}}
\tikzset{%
    adjunction/.style={%
        draw=none,
        every to/.append style={%
            edge node={node [sloped, allow upside down, auto=false]{$\dashv$}}}
    }
}

%% Used for extra wide diagrams, e.g. when the label is too large otherwise.
\tikzset{commutative diagrams/column sep/Huge/.initial=18ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% New environment for constructions.

%\expandafter\let\expandafter\oldproof\csname\string\proof\endcsname
%\let\oldendproof\endproof
\newenvironment{constr}{\begin{proof}[Construction]}{\end{proof}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% The following environment for desiderata should not be there. It is better
%%%% to use the issue tracker for desiderata.

\newenvironment{desiderata}{\begingroup\color{blue}\textbf{Desiderata.}}
{\endgroup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% The following piece of code from tex.stackexchange:
%%%%
%%%% http://tex.stackexchange.com/a/55180/14653
%%%%
%%%% We include it so that inference rules in align environments have enough
%%%% vertical space.

\newlength\minalignvsep

\def\align@preamble{%
   &\hfil
    \setboxz@h{\@lign$\m@th\displaystyle{##}$}%
    \ifnum\row@>\@ne
    \ifdim\ht\z@>\ht\strutbox@
    \dimen@\ht\z@
    \advance\dimen@\minalignvsep
    \ht\strutbox\dimen@
    \fi\fi
    \strut@
    \ifmeasuring@\savefieldlength@\fi
    \set@field
    \tabskip\z@skip
   &\setboxz@h{\@lign$\m@th\displaystyle{{}##}$}%
    \ifnum\row@>\@ne
    \ifdim\ht\z@>\ht\strutbox@
    \dimen@\ht\z@
    \advance\dimen@\minalignvsep
    \ht\strutbox@\dimen@
    \fi\fi
    \strut@
    \ifmeasuring@\savefieldlength@\fi
    \set@field
    \hfil
    \tabskip\alignsep@
}

\minalignvsep.2em

\allowdisplaybreaks

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setdescription[1]{itemsep=-0.2em}

\makeatother


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "hott-intro"
%%% End:

